From Voice to Value: Leveraging AI to Enhance Spoken Online Reviews on the Go

Online reviews help people make better decisions. Review platforms usually depend on typed input, where leaving a good review requires significant effort because users must carefully organize and articulate their thoughts. This may discourage users from leaving comprehensive and high-quality reviews, especially when they are on the go. To address this challenge, we developed Vocalizer, a mobile application that enables users to provide reviews through voice input, with enhancements from a large language model (LLM). In a longitudinal study, we analysed user interactions with the app, focusing on AI-driven features that help refine and improve reviews. Our findings show that users frequently utilized the AI agent to add more detailed information to their reviews. We also show how interactive AI features can improve users self-efficacy and willingness to share reviews online. Finally, we discuss the opportunities and challenges of integrating AI assistance into review-writing systems.

==> Drafts.tex <==
\begin{table}[ht]
\centering
\caption{User Satisfaction and AI Agent Utilization}
\label{tab:user_satisfaction}
\begin{tabular}{lccc}
\hline
AI Agent Usage & Useful & Satisfied & ShareReview \\
\hline
Once & 6.13 & 6.29 & 6.23 \\
Multiple Times & 6.36 & 6.27 & 5.82 \\
\hline
\end{tabular}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{RQ2.What linguistic constructs and communicative strategies do users employ when interacting with AI-powered review enhancement tools.}

\begin{itemize}
    \item \textbf {H2} User prompts that exhibit higher levels of lexical diversity, syntactic complexity, and semantic specificity will correlate with more accurate and comprehensive AI-generated review enhancements.
\end{itemize}

\textbf{RQ3.How do user characteristics and preferences influence the adoption and effectiveness of AI-powered review enhancement tools?}

==> TODO.tex <==
- Check review improvement ideas citations
- Technical image with voice and AI features up and down
- Check again reading one data
- Genarate high-quality images
- Check the hypothesis spelling in the second and last sections 
- Maybe they used imperative sentences to for sentiment and style chnages
- Some places we called 'users' and some places it is 'participant'
